Low-pass Personalized Subgraph Federated Recommendation

Federated Recommender Systems (FRS) preserve privacy by training decentralized models on client-specific user-item subgraphs without sharing raw data. However, FRS faces a unique challenge: subgraph structural imbalance, where drastic variations in subgraph scale (user/item counts) and connectivity (item degree) misalign client representations, making it challenging to train a robust model that respects each client's unique structural characteristics. To address this, we propose a Low-pass Personalized Subgraph Federated recommender system (LPSFed). LPSFed leverages graph Fourier transforms and low-pass spectral filtering to extract low-frequency structural signals that remain stable across subgraphs of varying size and degree, allowing robust personalized parameter updates guided by similarity to a neutral structural anchor. Additionally, we leverage a localized popularity bias-aware margin that captures item-degree imbalance within each subgraph and incorporates it into a personalized bias correction term to mitigate recommendation bias. Supported by theoretical analysis and validated on five real-world datasets, LPSFed achieves superior recommendation accuracy and enhances model robustness.

==> 3_relatedwork.tex <==
\section{Related Work}
FRS preserves privacy by decentralizing model training. The field has evolved from matrix factorization (FedMF~\citep{FedMF}) to personalized approaches (PFedRec~\citep{PFedRec}) and graph-based models that expand subgraphs on the server (FedPerGNN~\citep{FedPerGNN}). Spectral method (FedSSP~\citep{FedSSP}) has emerged in FL for graph and node classification to handle client heterogeneity, but existing approaches have been tailored to explicitly tackle the \textit{subgraph structural imbalance} in FRS and the \textit{localized popularity bias} it amplifies.
